Removing biased data to improve fairness and accuracy

Machine learning systems are often trained using data collected from historical decisions. If past decisions were biased, then automated systems that learn from historical data will also be biased. We propose a black-box approach to identify and remove biased training data. Machine learning models trained on such debiased data (a subset of the original training data) have low individual discrimination, often 0%. These models also have greater accuracy and lower statistical disparity than models trained on the full historical data. We evaluated our methodology in experiments using 6 real-world datasets. Our approach outperformed seven previous approaches in terms of individual discrimination and accuracy.

==> ls <==
\setlength{\belowcaptionskip}{-8pt}
\begin{figure*}
  \includegraphics[width=\textwidth]{algorithm-drawing.pdf}
  \vspace{-20pt}
  \caption{Flowchart with the steps in our approach. The left portion shows the steps in~\Cref{alg:rankpoints} 
  and the right portion shows the steps in~\Cref{alg:debiaseddata}. 
  The output of the algorithm is a debiased training data which can be used to 
  train a debiased model. \looseness=-1}
 \label{fig:algo-plot}
\end{figure*}

==> tables/correspond-real-accuracy_debiased.tex <==
D5 & 63 & \textbf{68} & 49 & 48 & 48 & 49 & 67 & \textbf{68}  \\ 


==> tables/correspond-real-accuracy_full.tex <==
D5 & 62 & 63 & 49 & 48 & 50 & 50 & \textbf{68} & 55  \\  


==> tables/discm_for_max_accuracy.tex <==
D1 & 2.1e+01 & 0.0 & 2.1e+01 & 7.3e-01 & 6.3e+00 & 4.5e+00 & 1.7e+01 & 6.6e-05  \\  
D2 & 1.2e+01 & 0.0 & 1.2e+01 & 1.8e+00 & 8.0e+00 & 4.2e-01 & 5.2e+00 & 9.3e-05  \\  
D3 & 1.1e+01 & 0.0 & 8.7e+00 & 1.1e+00 & 1.7e+00 & 5.6e-01 & 1.1e+01 & 7.0e-03  \\  
D4 & 9.4e-01 & 0.0 & 4.4e-01 & 8.5e-01 & 6.2e+00 & 1.7e+00 & 3.3e+00 & 3.1e-03  \\  
D5 & 9.4e-02 & 0.0 & 4.4e-02 & 6.4e-01 & 2.4e+00 & 4.4e-02 & 5.0e-01 & 1.6e-03  \\  
D6 & 5.0e-02 & 0.0 & 1.1e-02 & 2.8e-02 & 5.0e-01 & 3.0e+00 & 3.7e-02 & 1.3e-03  \\  
D7 & 1.4e+00 & 0.0 & 1.2e-01 & 7.7e-01 & 1.5e+00 & 2.8e+00 & 2.4e-01 & 0.0e+00  \\  
D8 & 1.9e-02 & 0.0 & 0.0e+00 & 1.9e-02 & 1.9e+01 & 6.8e+00 & 3.3e+01 & 0.0e+00  \\  \midrule


==> tables/discm_for_max_accuracy_dist10.tex <==
D1 & 2.0e+01 & 1.1e-01 & 2.1e+01 & 5.0e-01 & 6.2e+00 & 4.5e+00 & 1.7e+01 & 6.2e-01  \\  
D2 & 1.2e+01 & 2.2e-01 & 1.2e+01 & 1.8e+00 & 7.7e+00 & 8.1e-01 & 5.3e+00 & 8.9e-01  \\  
D3 & 1.1e+01 & 2.1e+00 & 8.7e+00 & 2.6e+00 & 2.7e+00 & 1.1e+00 & 1.1e+01 & 1.6e+00  \\  
D4 & 5.1e+00 & 4.8e+00 & 4.8e+00 & 4.9e+00 & 5.0e+00 & 2.8e+00 & 5.1e+00 & 2.7e+00  \\  
D5 & 5.8e-01 & 5.7e-01 & 6.5e-02 & 7.1e-01 & 2.6e+00 & 4.8e+00 & 6.1e-01 & 8.1e-05  \\  
D6 & 5.4e-02 & 6.0e-02 & 1.0e-02 & 1.1e-01 & 5.9e-01 & 5.4e+00 & 3.4e-02 & 2.1e-04  \\  
D7 & 2.0e+00 & 1.7e+00 & 6.2e-01 & 1.7e+00 & 2.1e+00 & 3.7e+00 & 2.6e-01 & 0.0e+00  \\  
D8 & 1.7e+00 & 1.3e+00 & 3.3e-02 & 1.5e+00 & 1.9e+01 & 7.3e+00 & 3.3e+01 & 0.0e+00  \\  \midrule


==> tables/discm_for_max_accuracy_dist10_floating.tex <==
D1 & 20.0 &  \textbf{0.11}  & 21.0 & 0.5 & 6.2 & 4.5 & 17.0 & 0.62 \\
D2 & 12.0 &  \textbf{0.22}  & 12.0 & 1.8 & 7.7 & 0.81 & 5.3 & 0.89 \\
D3 & 11.0 & 2.1 & 8.7 & 2.6 & 2.7 &  \textbf{1.1}  & 11.0 & 1.6 \\
D4 & 5.1 & 4.8 & 4.8 & 4.9 & 5.0 & 2.8 & 5.1 &  \textbf{2.7}  \\
D5 & 0.58 & 0.57 & 0.065 & 0.71 & 2.6 & 4.8 & 0.61 &  \textbf{8.1e$-$5}  \\
D6 & 0.054 & 0.06 & 0.01 & 0.11 & 0.59 & 5.4 & 0.034 &  \textbf{0.00021}  \\
D7 & 2.0 & 1.7 & 0.62 & 1.7 & 2.1 & 3.7 & 0.26 &  \textbf{0.0}  \\
D8 & 1.7 & 1.3 & 0.033 & 1.5 & 19.0 & 7.3 & 33.0 &  \textbf{0.0}  \\
\midrule
Avg. & 6.6 & 1.4 & 5.9 & 1.7 & 5.7 & 3.8 & 9.0 &  \textbf{0.73}  \\


==> tables/discm_for_max_accuracy_dist10_scientific.tex <==
D1 & 2.0e$+$1 &  \textbf{1.1e$-$1}  & 2.1e$+$1 & 5.0e$-$1 & 6.2e$+$0 & 4.5e$+$0 & 1.7e$+$1 & 6.2e$-$1 \\
D2 & 1.2e$+$1 &  \textbf{2.2e$-$1}  & 1.2e$+$1 & 1.8e$+$0 & 7.7e$+$0 & 8.1e$-$1 & 5.3e$+$0 & 8.9e$-$1 \\
D3 & 1.1e$+$1 & 2.1e$+$0 & 8.7e$+$0 & 2.6e$+$0 & 2.7e$+$0 &  \textbf{1.1e$+$0}  & 1.1e$+$1 & 1.6e$+$0 \\
D4 & 5.1e$+$0 & 4.8e$+$0 & 4.8e$+$0 & 4.9e$+$0 & 5.0e$+$0 & 2.8e$+$0 & 5.1e$+$0 &  \textbf{2.7e$+$0}  \\
D5 & 5.8e$-$1 & 5.7e$-$1 & 6.5e$-$2 & 7.1e$-$1 & 2.6e$+$0 & 4.8e$+$0 & 6.1e$-$1 &  \textbf{8.1e$-$5}  \\
D6 & 5.4e$-$2 & 6.0e$-$2 & 1.0e$-$2 & 1.1e$-$1 & 5.9e$-$1 & 5.4e$+$0 & 3.4e$-$2 &  \textbf{2.1e$-$4}  \\
D7 & 2.0e$+$0 & 1.7e$+$0 & 6.2e$-$1 & 1.7e$+$0 & 2.1e$+$0 & 3.7e$+$0 & 2.6e$-$1 &  \textbf{0.0}  \\
D8 & 1.7e$+$0 & 1.3e$+$0 & 3.3e$-$2 & 1.5e$+$0 & 1.9e$+$1 & 7.3e$+$0 & 3.3e$+$1 &  \textbf{0.0}  \\
\midrule
Avg. & 6.6e$+$0 & 1.4e$+$0 & 5.9e$+$0 & 1.7e$+$0 & 5.7e$+$0 & 3.8e$+$0 & 9.0e$+$0 &  \textbf{7.3e$-$1}  \\


==> tables/discm_for_max_accuracy_floating.tex <==
D1 & 21.0 &  \textbf{0.0}  & 21.0 & 0.73 & 6.3 & 4.5 & 17.0 & 6.6e$-$05 \\
D2 & 12.0 &  \textbf{0.0}  & 12.0 & 1.8 & 8.0 & 0.42 & 5.2 & 9.3e$-$05 \\
D3 & 11.0 &  \textbf{0.0}  & 8.7 & 1.1 & 1.7 & 0.56 & 11.0 & 0.007 \\
D4 & 0.94 &  \textbf{0.0}  & 0.44 & 0.85 & 6.2 & 1.7 & 3.3 & 0.0031 \\
D5 & 0.094 &  \textbf{0.0}  & 0.044 & 0.64 & 2.4 & 0.044 & 0.5 & 0.0016 \\
D6 & 0.05 &  \textbf{0.0}  & 0.011 & 0.028 & 0.5 & 3.0 & 0.037 & 0.0013 \\
D7 & 1.4 &  \textbf{0.0}  & 0.12 & 0.77 & 1.5 & 2.8 & 0.24 &  \textbf{0.0}  \\
D8 & 0.019 &  \textbf{0.0}  &  \textbf{0.0}  & 0.019 & 19.0 & 6.8 & 33.0 &  \textbf{0.0}  \\
\midrule
Avg. & 5.8 &  \textbf{0.0}  & 5.3 & 0.74 & 5.7 & 2.5 & 8.8 & 0.0016 \\


==> tables/discm_for_max_accuracy_scientific.tex <==
D1 & 2.1e$+$1 &  \textbf{0.0}  & 2.1e$+$1 & 7.3e$-$1 & 6.3e$+$0 & 4.5e$+$0 & 1.7e$+$1 & 6.6e$-$05 \\
D2 & 1.2e$+$1 &  \textbf{0.0}  & 1.2e$+$1 & 1.8e$+$0 & 8.0e$+$0 & 4.2e$-$1 & 5.2e$+$0 & 9.3e$-$05 \\
D3 & 1.1e$+$1 &  \textbf{0.0}  & 8.7e$+$0 & 1.1e$+$0 & 1.7e$+$0 & 5.6e$-$1 & 1.1e$+$1 & 7.0e$-$3 \\
D4 & 9.4e$-$1 &  \textbf{0.0}  & 4.4e$-$1 & 8.5e$-$1 & 6.2e$+$0 & 1.7e$+$0 & 3.3e$+$0 & 3.1e$-$3 \\
D5 & 9.4e$-$2 &  \textbf{0.0}  & 4.4e$-$2 & 6.4e$-$1 & 2.4e$+$0 & 4.4e$-$2 & 5.0e$-$1 & 1.6e$-$3 \\
D6 & 5.0e$-$2 &  \textbf{0.0}  & 1.1e$-$2 & 2.8e$-$2 & 5.0e$-$1 & 3.0e$+$0 & 3.7e$-$2 & 1.3e$-$3 \\
D7 & 1.4e$+$0 &  \textbf{0.0}  & 1.2e$-$1 & 7.7e$-$1 & 1.5e$+$0 & 2.8e$+$0 & 2.4e$-$1 &  \textbf{0.0}  \\
D8 & 1.9e$-$2 &  \textbf{0.0}  &  \textbf{0.0}  & 1.9e$-$2 & 1.9e$+$1 & 6.8e$+$0 & 3.3e$+$1 &  \textbf{0.0}  \\
\midrule
Avg. & 5.8e$+$0 &  \textbf{0.0}  & 5.3e$+$0 & 7.4e$-$1 & 5.7e$+$0 & 2.5e$+$0 & 8.8e$+$0 & 1.6e$-$3 \\


==> tables/discm_for_min_parity.tex <==
D1 & 2.0e+01 & 0.0 & 2.0e+01 & 1.0e-01 & 6.7e+00 & 5.2e+00 & 1.7e+01 & 2.2e-05  \\  
D2 & 1.3e+01 & 0.0 & 1.3e+01 & 1.8e+00 & 7.5e+00 & 2.5e-02 & 5.3e+00 & 4.2e-04  \\  
D3 & 7.6e+00 & 0.0 & 9.1e+00 & 2.0e+00 & 1.2e+00 & 3.9e-01 & 9.1e+00 & 2.4e-01  \\  
D4 & 3.9e+00 & 0.0 & 3.6e+00 & 1.2e+00 & 7.1e+00 & 5.5e+00 & 4.6e+00 & 4.6e-03  \\  
D5 & 8.5e-02 & 0.0 & 1.4e-02 & 2.4e-01 & 1.5e+00 & 0.0e+00 & 3.4e-01 & 5.9e-03  \\  
D6 & 4.9e-02 & 0.0 & 8.3e-03 & 3.2e-02 & 2.5e-01 & 4.1e-02 & 1.3e-02 & 2.1e-03  \\  
D7 & 1.2e+00 & 0.0 & 7.1e-02 & 9.8e-01 & 1.4e+00 & 0.0e+00 & 4.9e-01 & 0.0e+00  \\  
D8 & 1.0e+00 & 0.0 & 2.2e+00 & 3.8e-02 & 2.5e+01 & 0.0e+00 & 3.3e+01 & 0.0e+00  \\  \midrule


==> tables/discm_for_min_parity_dist10.tex <==
D1 & 2.0e+01 & 1.1e-01 & 2.0e+01 & 1.0e-01 & 6.7e+00 & 5.2e+00 & 1.7e+01 & 7.5e-01  \\  
D2 & 1.3e+01 & 2.2e-01 & 1.3e+01 & 1.8e+00 & 7.5e+00 & 1.1e+00 & 5.3e+00 & 1.2e+00  \\  
D3 & 7.8e+00 & 2.6e+00 & 9.1e+00 & 3.0e+00 & 3.3e+00 & 1.5e+00 & 9.5e+00 & 2.8e+00  \\  
D4 & 6.0e+00 & 5.3e+00 & 5.9e+00 & 5.4e+00 & 7.2e+00 & 5.9e+00 & 6.2e+00 & 4.2e+00  \\  
D5 & 3.2e-01 & 4.1e-01 & 2.1e-02 & 2.8e-01 & 1.7e+00 & 0.0e+00 & 3.8e-01 & 9.8e-05  \\  
D6 & 5.2e-02 & 6.1e-02 & 8.8e-03 & 5.8e-02 & 3.1e-01 & 4.6e-01 & 1.4e-02 & 2.3e-04  \\  
D7 & 2.1e+00 & 1.9e+00 & 4.6e-01 & 1.9e+00 & 2.2e+00 & 0.0e+00 & 6.5e-01 & 0.0e+00  \\  
D8 & 1.7e+00 & 1.3e+00 & 2.2e+00 & 1.5e+00 & 2.5e+01 & 0.0e+00 & 3.3e+01 & 8.6e-01  \\  \midrule


==> tables/discm_for_min_parity_dist10_floating.tex <==
D1 & 20.0 & 0.11 & 20.0 &  \textbf{0.1}  & 6.7 & 5.2 & 17.0 & 0.75 \\
D2 & 13.0 &  \textbf{0.22}  & 13.0 & 1.8 & 7.5 & 1.1 & 5.3 & 1.2 \\
D3 & 7.8 & 2.6 & 9.1 & 3.0 & 3.3 &  \textbf{1.5}  & 9.5 & 2.8 \\
D4 & 6.0 & 5.3 & 5.9 & 5.4 & 7.2 & 5.9 & 6.2 &  \textbf{4.2}  \\
D5 & 0.32 & 0.41 & 0.021 & 0.28 & 1.7 &  \textbf{0.0}  & 0.38 & 9.8e$-$5 \\
D6 & 0.052 & 0.061 & 0.0088 & 0.058 & 0.31 & 0.46 & 0.014 &  \textbf{0.00023}  \\
D7 & 2.1 & 1.9 & 0.46 & 1.9 & 2.2 &  \textbf{0.0}  & 0.65 &  \textbf{0.0}  \\
D8 & 1.7 & 1.3 & 2.2 & 1.5 & 25.0 &  \textbf{0.0}  & 33.0 & 0.86 \\
\midrule
Avg. & 6.4 & 1.5 & 6.3 & 1.8 & 6.7 & 1.8 & 9.0 &  \textbf{1.2}  \\


==> tables/discm_for_min_parity_dist10_scientific.tex <==
D1 & 2.0e$+$1 & 1.1e$-$1 & 2.0e$+$1 &  \textbf{1.0e$-$1}  & 6.7e$+$0 & 5.2e$+$0 & 1.7e$+$1 & 7.5e$-$1 \\
D2 & 1.3e$+$1 &  \textbf{2.2e$-$1}  & 1.3e$+$1 & 1.8e$+$0 & 7.5e$+$0 & 1.1e$+$0 & 5.3e$+$0 & 1.2e$+$0 \\
D3 & 7.8e$+$0 & 2.6e$+$0 & 9.1e$+$0 & 3.0e$+$0 & 3.3e$+$0 &  \textbf{1.5e$+$0}  & 9.5e$+$0 & 2.8e$+$0 \\
D4 & 6.0e$+$0 & 5.3e$+$0 & 5.9e$+$0 & 5.4e$+$0 & 7.2e$+$0 & 5.9e$+$0 & 6.2e$+$0 &  \textbf{4.2e$+$0}  \\
D5 & 3.2e$-$1 & 4.1e$-$1 & 2.1e$-$2 & 2.8e$-$1 & 1.7e$+$0 &  \textbf{0.0}  & 3.8e$-$1 & 9.8e$-$5 \\
D6 & 5.2e$-$2 & 6.1e$-$2 & 8.8e$-$3 & 5.8e$-$2 & 3.1e$-$1 & 4.6e$-$1 & 1.4e$-$2 &  \textbf{2.3e$-$4}  \\
D7 & 2.1e$+$0 & 1.9e$+$0 & 4.6e$-$1 & 1.9e$+$0 & 2.2e$+$0 &  \textbf{0.0}  & 6.5e$-$1 &  \textbf{0.0}  \\
D8 & 1.7e$+$0 & 1.3e$+$0 & 2.2e$+$0 & 1.5e$+$0 & 2.5e$+$1 &  \textbf{0.0}  & 3.3e$+$1 & 8.6e$-$1 \\
\midrule
Avg. & 6.4e$+$0 & 1.5e$+$0 & 6.3e$+$0 & 1.8e$+$0 & 6.7e$+$0 & 1.8e$+$0 & 9.0e$+$0 &  \textbf{1.2e$+$0}  \\


==> tables/discm_for_min_parity_floating.tex <==
D1 & 20.0 &  \textbf{0.0}  & 20.0 & 0.1 & 6.7 & 5.2 & 17.0 & 2.2e$-$05 \\
D2 & 13.0 &  \textbf{0.0}  & 13.0 & 1.8 & 7.5 & 0.025 & 5.3 & 0.00042 \\
D3 & 7.6 &  \textbf{0.0}  & 9.1 & 2.0 & 1.2 & 0.39 & 9.1 & 0.24 \\
D4 & 3.9 &  \textbf{0.0}  & 3.6 & 1.2 & 7.1 & 5.5 & 4.6 & 0.0046 \\
D5 & 0.085 &  \textbf{0.0}  & 0.014 & 0.24 & 1.5 &  \textbf{0.0}  & 0.34 & 0.0059 \\
D6 & 0.049 &  \textbf{0.0}  & 0.0083 & 0.032 & 0.25 & 0.041 & 0.013 & 0.0021 \\
D7 & 1.2 &  \textbf{0.0}  & 0.071 & 0.98 & 1.4 &  \textbf{0.0}  & 0.49 &  \textbf{0.0}  \\
D8 & 1.0 &  \textbf{0.0}  & 2.2 & 0.038 & 25.0 &  \textbf{0.0}  & 33.0 &  \textbf{0.0}  \\
\midrule
Avg. & 5.9 &  \textbf{0.0}  & 6.0 & 0.8 & 6.3 & 1.4 & 8.7 & 0.032 \\


==> tables/discm_for_min_parity_scientific.tex <==
D1 & 2.0e$+$1 &  \textbf{0.0}  & 2.0e$+$1 & 1.0e$-$1 & 6.7e$+$0 & 5.2e$+$0 & 1.7e$+$1 & 2.2e$-$05 \\
D2 & 1.3e$+$1 &  \textbf{0.0}  & 1.3e$+$1 & 1.8e$+$0 & 7.5e$+$0 & 2.5e$-$2 & 5.3e$+$0 & 4.2e$-$4 \\
D3 & 7.6e$+$0 &  \textbf{0.0}  & 9.1e$+$0 & 2.0e$+$0 & 1.2e$+$0 & 3.9e$-$1 & 9.1e$+$0 & 2.4e$-$1 \\
D4 & 3.9e$+$0 &  \textbf{0.0}  & 3.6e$+$0 & 1.2e$+$0 & 7.1e$+$0 & 5.5e$+$0 & 4.6e$+$0 & 4.6e$-$3 \\
D5 & 8.5e$-$2 &  \textbf{0.0}  & 1.4e$-$2 & 2.4e$-$1 & 1.5e$+$0 &  \textbf{0.0}  & 3.4e$-$1 & 5.9e$-$3 \\
D6 & 4.9e$-$2 &  \textbf{0.0}  & 8.3e$-$3 & 3.2e$-$2 & 2.5e$-$1 & 4.1e$-$2 & 1.3e$-$2 & 2.1e$-$3 \\
D7 & 1.2e$+$0 &  \textbf{0.0}  & 7.1e$-$2 & 9.8e$-$1 & 1.4e$+$0 &  \textbf{0.0}  & 4.9e$-$1 &  \textbf{0.0}  \\
D8 & 1.0e$+$0 &  \textbf{0.0}  & 2.2e$+$0 & 3.8e$-$2 & 2.5e$+$1 &  \textbf{0.0}  & 3.3e$+$1 &  \textbf{0.0}  \\
\midrule
Avg. & 5.9e$+$0 &  \textbf{0.0}  & 6.0e$+$0 & 8.0e$-$1 & 6.3e$+$0 & 1.4e$+$0 & 8.7e$+$0 & 3.2e$-$2 \\


==> tables/max-accuracy-model_dist10_scientific.tex <==
D1 & 2.0e$+$1 &  \textbf{1.1e$-$1}  & 2.1e$+$1 & 5.0e$-$1 & 6.2e$+$0 & 4.5e$+$0 & 1.7e$+$1 & 6.2e$-$1 
& 82 & 84 & 82 & 85 & 82 & 85 & 85 &  \textbf{86}  
& 29 & 13 & 29 & 11 & 1.5 & 3.3 &  \textbf{0.18}  & 12 \\
D2 & 1.2e$+$1 &  \textbf{2.2e$-$1}  & 1.2e$+$1 & 1.8e$+$0 & 7.7e$+$0 & 8.1e$-$1 & 5.3e$+$0 & 8.9e$-$1 
& 80 & 81 & 81 & 81 & 81 & 80 &  \textbf{87}  & 82 
& 22 & 13 & 21 & 11 & 5.4 &  \textbf{0.18}  & 0.37 & 14 \\
D3 & 1.1e$+$1 & 2.1e$+$0 & 8.7e$+$0 & 2.6e$+$0 & 2.7e$+$0 &  \textbf{1.1e$+$0}  & 1.1e$+$1 & 1.6e$+$0 
& 82 & 82 & 81 & 83 &  \textbf{85}  & 78 & 83 & 82 
& 11 & 3.1 & 6.1 & 3.2 &  \textbf{1.2}  & 2.6 & 5 & 5.8 \\
D4 & 5.1e$+$0 & 4.8e$+$0 & 4.8e$+$0 & 4.9e$+$0 & 5.0e$+$0 & 2.8e$+$0 & 5.1e$+$0 &  \textbf{2.7e$+$0}  
&  \textbf{100}  &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  & 96 &  \textbf{100}  &  \textbf{100}  
& 18 & 5.7 & 20 &  \textbf{2.4}  & 8 & 16 & 12 & 16 \\
D5 & 5.8e$-$1 & 5.7e$-$1 & 6.5e$-$2 & 7.1e$-$1 & 2.6e$+$0 & 4.8e$+$0 & 6.1e$-$1 &  \textbf{8.1e$-$5}  
& 75 & 74 & 74 & 55 & 75 & 87 & 67 &  \textbf{100}  
& 32 & 26 & 38 & 3.9 &  \textbf{1.6}  & 21 & 22 & 28 \\
D6 & 5.4e$-$2 & 6.0e$-$2 & 1.0e$-$2 & 1.1e$-$1 & 5.9e$-$1 & 5.4e$+$0 & 3.4e$-$2 &  \textbf{2.1e$-$4}  
& 66 & 74 & 50 & 70 & 82 & 81 & 75 &  \textbf{100}  
& 38 & 25 & 48 & 15 &  \textbf{0.078}  & 22 & 26 & 19 \\
D7 & 2.0e$+$0 & 1.7e$+$0 & 6.2e$-$1 & 1.7e$+$0 & 2.1e$+$0 & 3.7e$+$0 & 2.6e$-$1 &  \textbf{0.0}  
& 78 & 78 & 75 & 79 & 78 &  \textbf{87}  & 85 & 83 
& 13 & 6.1 & 9 & 2.1 &  \textbf{1.2}  & 2 & 2.3 & 12 \\
D8 & 1.7e$+$0 & 1.3e$+$0 & 3.3e$-$2 & 1.5e$+$0 & 1.9e$+$1 & 7.3e$+$0 & 3.3e$+$1 &  \textbf{0.0}  
&  \textbf{100}  &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  & 75 &  \textbf{100}  
& 11 & 11 & 10 & 10 &  \textbf{0.0}  & 12 &  \textbf{0.0}  & 10 \\
\midrule
Avg. & 6.6e$+$0 & 1.4e$+$0 & 5.9e$+$0 & 1.7e$+$0 & 5.7e$+$0 & 3.8e$+$0 & 9.0e$+$0 &  \textbf{7.3e$-$1}  
& 82 & 84 & 80 & 81 & 85 & 86 & 82 &  \textbf{91}  
& 22 & 13 & 23 & 7.3 &  \textbf{2.4}  & 9.9 & 8.5 & 15 \\


==> tables/max-accuracy-model_scientific.tex <==
D1 & 2.1e$+$1 &  \textbf{0.0}  & 2.1e$+$1 & 7.3e$-$1 & 6.3e$+$0 & 4.5e$+$0 & 1.7e$+$1 & 6.6e$-$05 
& 82 & 82 & 82 & 82 & 82 & 83 & 85 &  \textbf{93}  
& 29 & 13 & 29 & 11 & 1.5 & 3.3 &  \textbf{0.18}  & 9.9 \\
D2 & 1.2e$+$1 &  \textbf{0.0}  & 1.2e$+$1 & 1.8e$+$0 & 8.0e$+$0 & 4.2e$-$1 & 5.2e$+$0 & 9.3e$-$05 
& 85 & 85 & 85 & 85 & 85 & 85 & 88 &  \textbf{92}  
& 22 & 13 & 21 & 11 & 5.4 &  \textbf{0.18}  & 0.37 & 13 \\
D3 & 1.1e$+$1 &  \textbf{0.0}  & 8.7e$+$0 & 1.1e$+$0 & 1.7e$+$0 & 5.6e$-$1 & 1.1e$+$1 & 7.0e$-$3 
& 82 & 82 & 81 & 83 &  \textbf{85}  & 78 & 82 & 82 
& 11 & 3.1 & 6.1 & 3.2 &  \textbf{1.2}  & 2.6 & 5 & 7.9 \\
D4 & 9.4e$-$1 &  \textbf{0.0}  & 4.4e$-$1 & 8.5e$-$1 & 6.2e$+$0 & 1.7e$+$0 & 3.3e$+$0 & 3.1e$-$3 
& 98 & 98 & 98 &  \textbf{99}  & 98 & 89 & 96 & 98 
& 18 & 5.7 & 20 &  \textbf{2.4}  & 8 & 16 & 12 & 17 \\
D5 & 9.4e$-$2 &  \textbf{0.0}  & 4.4e$-$2 & 6.4e$-$1 & 2.4e$+$0 & 4.4e$-$2 & 5.0e$-$1 & 1.6e$-$3 
& 77 & 77 & 72 & 61 & 85 & 87 & 80 &  \textbf{100}  
& 32 & 26 & 38 & 3.9 &  \textbf{1.6}  & 21 & 22 & 26 \\
D6 & 5.0e$-$2 &  \textbf{0.0}  & 1.1e$-$2 & 2.8e$-$2 & 5.0e$-$1 & 3.0e$+$0 & 3.7e$-$2 & 1.3e$-$3 
& 74 & 81 & 50 & 76 & 87 & 83 & 81 &  \textbf{100}  
& 38 & 25 & 48 & 15 &  \textbf{0.078}  & 22 & 26 & 26 \\
D7 & 1.4e$+$0 &  \textbf{0.0}  & 1.2e$-$1 & 7.7e$-$1 & 1.5e$+$0 & 2.8e$+$0 & 2.4e$-$1 &  \textbf{0.0}  
& 78 & 78 & 75 & 78 & 78 &  \textbf{85}  &  \textbf{85}  & 80 
& 13 & 6.1 & 9 & 2.1 &  \textbf{1.2}  & 2 & 2.3 & 3.4 \\
D8 & 1.9e$-$2 &  \textbf{0.0}  &  \textbf{0.0}  & 1.9e$-$2 & 1.9e$+$1 & 6.8e$+$0 & 3.3e$+$1 &  \textbf{0.0}  
&  \textbf{100}  &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  & 75 &  \textbf{100}  
& 11 & 11 & 10 & 10 &  \textbf{0.0}  & 12 &  \textbf{0.0}  & 10 \\
\midrule
Avg. & 5.8e$+$0 &  \textbf{0.0}  & 5.3e$+$0 & 7.4e$-$1 & 5.7e$+$0 & 2.5e$+$0 & 8.8e$+$0 & 1.6e$-$3 
& 84 & 85 & 80 & 83 & 87 & 86 & 84 &  \textbf{93}  
& 22 & 13 & 23 & 7.3 &  \textbf{2.4}  & 9.9 & 8.5 & 14 \\


==> tables/max-real-accuracy_debiased.tex <==
D5 & 6.3e+01 & 6.8e+01 & 5.2e+01 & 5.1e+01 & 5.2e+01 & 5.3e+01 & 7.4e+01 & 6.8e+01  \\  \hline


==> tables/max-real-accuracy_full.tex <==
D5 & 6.2e+01 & 6.3e+01 & 5.0e+01 & 5.1e+01 & 5.1e+01 & 5.1e+01 & 6.9e+01 & 5.5e+01  \\  \hline


==> tables/max-test-accuracy.tex <==
D1 & 82 & 82 & 82 & 82 & 82 & 83 & 85 &  \textbf{93}  \\
D2 & 85 & 85 & 85 & 85 & 85 & 85 & 88 &  \textbf{92}  \\
D3 & 82 & 82 & 81 & 83 &  \textbf{85}  & 78 & 82 & 82 \\
D4 & 98 & 98 & 98 &  \textbf{99}  & 98 & 89 & 96 & 98 \\
D5 & 77 & 77 & 72 & 61 & 85 & 87 & 80 &  \textbf{100}  \\
D6 & 74 & 81 & 50 & 76 & 87 & 83 & 81 &  \textbf{100}  \\
D7 & 78 & 78 & 75 & 78 & 78 &  \textbf{85}  &  \textbf{85}  & 80 \\
D8 &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  & 75 &  \textbf{100}  \\
\midrule
Avg. & 84 & 85 & 80 & 83 & 87 & 86 & 84 &  \textbf{93}  \\


==> tables/max-test-accuracy_dist10.tex <==
D1 & 82 & 84 & 82 & 85 & 82 & 85 & 85 &  \textbf{86}  \\
D2 & 80 & 81 & 81 & 81 & 81 & 80 &  \textbf{87}  & 82 \\
D3 & 82 & 82 & 81 & 83 &  \textbf{85}  & 78 & 83 & 82 \\
D4 &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  & 96 &  \textbf{100}  &  \textbf{100}  \\
D5 & 75 & 74 & 74 & 55 & 75 & 87 & 67 &  \textbf{100}  \\
D6 & 66 & 74 & 50 & 70 & 82 & 81 & 75 &  \textbf{100}  \\
D7 & 78 & 78 & 75 & 79 & 78 &  \textbf{87}  & 85 & 83 \\
D8 &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  & 75 &  \textbf{100}  \\
\midrule
Avg. & 82 & 84 & 80 & 81 & 85 & 86 & 82 &  \textbf{91}  \\


==> tables/mean-test-accuracy.tex <==
D1 & 4.3e+01 & 8.1e+01 & 8.2e+01 & 8.0e+01 & 8.2e+01 & 8.1e+01 & \textbf{9.1e+01}  \\  \hline
D2 & 6.4e+01 & 7.6e+01 & 7.6e+01 & 7.7e+01 & 6.8e+01 & 7.3e+01 & \textbf{7.7e+01}  \\  \hline
D3 & 5.3e+01 & 9.3e+01 & 9.5e+01 & 9.2e+01 & 7.8e+01 & 8.7e+01 & \textbf{9.5e+01}  \\  \hline
D4 & 4.4e+01 & 6.6e+01 & 4.9e+01 & 8.1e+01 & 8.3e+01 & 6.7e+01 & \textbf{9.4e+01}  \\  \hline
D5 & 4.7e+01 & 6.3e+01 & 7.0e+01 & 8.2e+01 & 7.8e+01 & 7.5e+01 & \textbf{9.8e+01}  \\  \hline
D6 & 5.2e+01 & 7.2e+01 & 7.6e+01 & 7.6e+01 & 8.3e+01 & 8.1e+01 & \textbf{7.6e+01}  \\  


==> tables/min-discm-model_dist10_scientific.tex <==
D1 & 1.9e$+$1 &  \textbf{2.6e$-$3}  & 1.9e$+$1 & 4.2e$-$2 & 5.6e$+$0 & 4.1e$-$1 & 1.2e$+$1 & 6.2e$-$1 
& 81 & 83 & 81 & 85 & 81 & 84 & 85 &  \textbf{86}  
& 29 & 15 & 28 & 8.9 & 3.3 & 3.6 &  \textbf{2.3}  & 9.8 \\
D2 & 1.1e$+$1 &  \textbf{4.4e$-$4}  & 1.1e$+$1 & 4.5e$-$1 & 6.0e$+$0 & 3.7e$-$1 & 4.3e$+$0 & 6.7e$-$1 
& 79 & 80 & 80 & 80 & 79 & 80 &  \textbf{85}  & 81 
& 21 & 8.1 & 20 & 12 & 7 &  \textbf{0.59}  & 7.8 & 12 \\
D3 & 6.4e$+$0 & 1.9e$+$0 & 4.2e$+$0 & 2.2e$+$0 & 2.0e$+$0 &  \textbf{6.6e$-$2}  & 8.7e$+$0 & 1.6e$+$0 
& 75 & 81 & 74 & 73 & 76 & 62 & 76 &  \textbf{82}  
& 1.6 &  \textbf{1.1}  & 2.1 & 2.1 & 3.3 & 2.7 & 1.5 & 7.6 \\
D4 & 4.7e$+$0 & 4.6e$+$0 & 4.8e$+$0 & 4.7e$+$0 & 4.2e$+$0 &  \textbf{8.7e$-$1}  & 4.5e$+$0 & 2.3e$+$0 
& 99 & 98 &  \textbf{100}  & 98 & 96 & 90 & 98 & 97 
& 13 & 12 & 6.6 & 13 & 12 & 5.4 & 11 &  \textbf{4.4}  \\
D5 & 1.9e$-$1 & 2.0e$-$1 & 5.2e$-$3 & 1.4e$-$1 & 9.7e$-$1 &  \textbf{0.0}  & 3.6e$-$1 & 8.1e$-$5 
& 63 & 62 & 60 & 44 & 63 & 70 & 64 &  \textbf{100}  
& 26 & 24 & 33 & 2.4 & 3.7 &  \textbf{0.0}  & 8.4 & 0.72 \\
D6 & 4.8e$-$2 & 4.6e$-$2 & 3.3e$-$3 & 3.3e$-$2 & 2.1e$-$1 & 1.8e$-$1 & 8.8e$-$3 &  \textbf{2.0e$-$4}  
& 60 & 67 & 49 & 59 & 72 & 72 & 67 &  \textbf{99}  
& 38 & 23 & 47 & 14 &  \textbf{1.1}  & 21 & 26 & 26 \\
D7 & 1.8e$+$0 & 1.6e$+$0 & 1.9e$-$1 & 1.5e$+$0 & 1.9e$+$0 &  \textbf{0.0}  & 7.9e$-$2 &  \textbf{0.0}  
& 76 & 76 & 71 & 76 & 75 &  \textbf{86}  & 85 & 83 
& 12 & 4.7 & 11 & 1.4 & 4.6 &  \textbf{0.0}  & 3.4 & 6.5 \\
D8 & 1.7e$+$0 & 1.3e$+$0 & 3.3e$-$2 & 1.5e$+$0 & 1.9e$+$1 &  \textbf{0.0}  & 3.3e$+$1 &  \textbf{0.0}  
&  \textbf{100}  &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  & 57 & 75 &  \textbf{100}  
&  \textbf{0.0}  &  \textbf{0.0}  & 30 &  \textbf{0.0}  & 50 &  \textbf{0.0}  &  \textbf{0.0}  & 30 \\
\midrule
Avg. & 5.6e$+$0 & 1.2e$+$0 & 4.9e$+$0 & 1.3e$+$0 & 5.0e$+$0 &  \textbf{2.4e$-$1}  & 7.9e$+$0 & 6.5e$-$1 
& 79 & 80 & 76 & 76 & 80 & 75 & 79 &  \textbf{91}  
& 18 & 11 & 22 & 6.7 & 11 &  \textbf{4.2}  & 7.5 & 12 \\


==> tables/min-discm-model_scientific.tex <==
D1 & 1.9e$+$1 &  \textbf{0.0}  & 1.9e$+$1 & 6.4e$-$3 & 5.7e$+$0 & 9.6e$-$2 & 1.2e$+$1 &  \textbf{0.0}  
& 80 & 82 & 80 & 81 & 80 & 81 & 85 &  \textbf{92}  
& 29 & 13 & 28 & 8.7 & 3.3 & 3.6 &  \textbf{2.3}  & 7.8 \\
D2 & 1.1e$+$1 &  \textbf{0.0}  & 1.1e$+$1 & 3.8e$-$1 & 6.0e$+$0 & 6.3e$-$3 & 4.3e$+$0 &  \textbf{0.0}  
& 83 & 85 & 84 & 84 & 83 & 84 & 87 &  \textbf{92}  
& 21 & 13 & 20 & 12 & 7 &  \textbf{0.33}  & 7.8 & 10 \\
D3 & 6.2e$+$0 &  \textbf{0.0}  & 3.8e$+$0 & 1.4e$-$2 & 8.3e$-$2 &  \textbf{0.0}  & 8.1e$+$0 &  \textbf{0.0}  
& 75 &  \textbf{82}  & 74 & 73 & 75 & 62 & 76 & 81 
& 1.6 & 3.1 & 2.1 & 14 & 6.2 &  \textbf{0.085}  & 1.5 & 9.8 \\
D4 & 1.5e$-$3 &  \textbf{0.0}  & 2.0e$-$2 &  \textbf{0.0}  & 3.5e$+$0 & 3.7e$-$2 & 2.3e$+$0 &  \textbf{0.0}  
& 96 &  \textbf{98}  & 95 & 92 & 92 & 69 & 92 & 96 
& 15 & 5.7 & 20 & 12 & 13 &  \textbf{3.8}  & 11 & 25 \\
D5 & 1.3e$-$2 &  \textbf{0.0}  & 4.6e$-$3 & 1.1e$-$1 & 8.7e$-$1 &  \textbf{0.0}  & 3.4e$-$1 &  \textbf{0.0}  
& 73 &  \textbf{77}  & 62 & 48 & 76 & 73 & 76 & 74 
& 21 & 26 & 33 & 2.3 & 3.7 &  \textbf{0.0}  & 0.96 & 25 \\
D6 & 4.5e$-$2 &  \textbf{0.0}  & 4.6e$-$3 & 2.0e$-$2 & 1.6e$-$1 & 9.8e$-$4 & 1.0e$-$2 &  \textbf{0.0}  
& 67 & 81 & 49 & 65 & 78 & 78 & 79 &  \textbf{84}  
& 39 & 25 & 49 & 14 &  \textbf{1.1}  & 22 & 26 & 23 \\
D7 & 1.2e$+$0 &  \textbf{0.0}  & 4.0e$-$2 & 6.5e$-$1 & 1.3e$+$0 &  \textbf{0.0}  & 4.6e$-$2 &  \textbf{0.0}  
& 76 & 78 & 71 & 77 & 75 & 83 &  \textbf{85}  & 80 
& 12 & 6.1 & 11 & 1.6 & 4.6 &  \textbf{0.0}  & 3.4 & 0.12 \\
D8 & 1.9e$-$2 &  \textbf{0.0}  &  \textbf{0.0}  & 1.9e$-$2 & 1.9e$+$1 &  \textbf{0.0}  & 3.3e$+$1 &  \textbf{0.0}  
&  \textbf{100}  &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  & 50 & 75 &  \textbf{100}  
& 33 & 11 & 12 & 22 & 50 &  \textbf{0.0}  &  \textbf{0.0}  &  \textbf{0.0}  \\
\midrule
Avg. & 4.7e$+$0 &  \textbf{0.0}  & 4.2e$+$0 & 1.5e$-$1 & 4.6e$+$0 & 1.8e$-$2 & 7.5e$+$0 &  \textbf{0.0}  
& 81 & 85 & 76 & 77 & 82 & 72 & 81 &  \textbf{87}  
& 21 & 13 & 22 & 11 & 11 &  \textbf{3.7}  & 6.6 & 13 \\


==> tables/min-discm.tex <==
D1 & 1.9e+01 & 0.0 & 1.9e+01 & 6.4e-03 & 5.7e+00 & 9.6e-02 & 1.2e+01 & 0.0e+00  \\  
D2 & 1.1e+01 & 0.0 & 1.1e+01 & 3.8e-01 & 6.0e+00 & 6.3e-03 & 4.3e+00 & 0.0e+00  \\  
D3 & 6.2e+00 & 0.0 & 3.8e+00 & 1.4e-02 & 8.3e-02 & 0.0e+00 & 8.1e+00 & 0.0e+00  \\  
D4 & 1.5e-03 & 0.0 & 2.0e-02 & 0.0e+00 & 3.5e+00 & 3.7e-02 & 2.3e+00 & 0.0e+00  \\  
D5 & 1.3e-02 & 0.0 & 4.6e-03 & 1.1e-01 & 8.7e-01 & 0.0e+00 & 3.4e-01 & 0.0e+00  \\  
D6 & 4.5e-02 & 0.0 & 4.6e-03 & 2.0e-02 & 1.6e-01 & 9.8e-04 & 1.0e-02 & 0.0e+00  \\  
D7 & 1.2e+00 & 0.0 & 4.0e-02 & 6.5e-01 & 1.3e+00 & 0.0e+00 & 4.6e-02 & 0.0e+00  \\  
D8 & 1.9e-02 & 0.0 & 0.0e+00 & 1.9e-02 & 1.9e+01 & 0.0e+00 & 3.3e+01 & 0.0e+00  \\  \midrule


==> tables/min-discm_dist10.tex <==
D1 & 1.9e+01 & 2.6e-03 & 1.9e+01 & 4.2e-02 & 5.6e+00 & 4.1e-01 & 1.2e+01 & 6.2e-01  \\  
D2 & 1.1e+01 & 4.4e-04 & 1.1e+01 & 4.5e-01 & 6.0e+00 & 3.7e-01 & 4.3e+00 & 6.7e-01  \\  
D3 & 6.4e+00 & 1.9e+00 & 4.2e+00 & 2.2e+00 & 2.0e+00 & 6.6e-02 & 8.7e+00 & 1.6e+00  \\  
D4 & 4.7e+00 & 4.6e+00 & 4.8e+00 & 4.7e+00 & 4.2e+00 & 8.7e-01 & 4.5e+00 & 2.3e+00  \\  
D5 & 1.9e-01 & 2.0e-01 & 5.2e-03 & 1.4e-01 & 9.7e-01 & 0.0e+00 & 3.6e-01 & 8.1e-05  \\  
D6 & 4.8e-02 & 4.6e-02 & 3.3e-03 & 3.3e-02 & 2.1e-01 & 1.8e-01 & 8.8e-03 & 2.0e-04  \\  
D7 & 1.8e+00 & 1.6e+00 & 1.9e-01 & 1.5e+00 & 1.9e+00 & 0.0e+00 & 7.9e-02 & 0.0e+00  \\  
D8 & 1.7e+00 & 1.3e+00 & 3.3e-02 & 1.5e+00 & 1.9e+01 & 0.0e+00 & 3.3e+01 & 0.0e+00  \\  \midrule


==> tables/min-discm_dist10_floating.tex <==
D1 & 19.0 &  \textbf{0.0026}  & 19.0 & 0.042 & 5.6 & 0.41 & 12.0 & 0.62 \\
D2 & 11.0 &  \textbf{0.00044}  & 11.0 & 0.45 & 6.0 & 0.37 & 4.3 & 0.67 \\
D3 & 6.4 & 1.9 & 4.2 & 2.2 & 2.0 &  \textbf{0.066}  & 8.7 & 1.6 \\
D4 & 4.7 & 4.6 & 4.8 & 4.7 & 4.2 &  \textbf{0.87}  & 4.5 & 2.3 \\
D5 & 0.19 & 0.2 & 0.0052 & 0.14 & 0.97 &  \textbf{0.0}  & 0.36 & 8.1e$-$5 \\
D6 & 0.048 & 0.046 & 0.0033 & 0.033 & 0.21 & 0.18 & 0.0088 &  \textbf{0.0002}  \\
D7 & 1.8 & 1.6 & 0.19 & 1.5 & 1.9 &  \textbf{0.0}  & 0.079 &  \textbf{0.0}  \\
D8 & 1.7 & 1.3 & 0.033 & 1.5 & 19.0 &  \textbf{0.0}  & 33.0 &  \textbf{0.0}  \\
\midrule
Avg. & 5.6 & 1.2 & 4.9 & 1.3 & 5.0 &  \textbf{0.24}  & 7.9 & 0.65 \\


==> tables/min-discm_dist10_scientific.tex <==
D1 & 1.9e$+$1 &  \textbf{2.6e$-$3}  & 1.9e$+$1 & 4.2e$-$2 & 5.6e$+$0 & 4.1e$-$1 & 1.2e$+$1 & 6.2e$-$1 \\
D2 & 1.1e$+$1 &  \textbf{4.4e$-$4}  & 1.1e$+$1 & 4.5e$-$1 & 6.0e$+$0 & 3.7e$-$1 & 4.3e$+$0 & 6.7e$-$1 \\
D3 & 6.4e$+$0 & 1.9e$+$0 & 4.2e$+$0 & 2.2e$+$0 & 2.0e$+$0 &  \textbf{6.6e$-$2}  & 8.7e$+$0 & 1.6e$+$0 \\
D4 & 4.7e$+$0 & 4.6e$+$0 & 4.8e$+$0 & 4.7e$+$0 & 4.2e$+$0 &  \textbf{8.7e$-$1}  & 4.5e$+$0 & 2.3e$+$0 \\
D5 & 1.9e$-$1 & 2.0e$-$1 & 5.2e$-$3 & 1.4e$-$1 & 9.7e$-$1 &  \textbf{0.0}  & 3.6e$-$1 & 8.1e$-$5 \\
D6 & 4.8e$-$2 & 4.6e$-$2 & 3.3e$-$3 & 3.3e$-$2 & 2.1e$-$1 & 1.8e$-$1 & 8.8e$-$3 &  \textbf{2.0e$-$4}  \\
D7 & 1.8e$+$0 & 1.6e$+$0 & 1.9e$-$1 & 1.5e$+$0 & 1.9e$+$0 &  \textbf{0.0}  & 7.9e$-$2 &  \textbf{0.0}  \\
D8 & 1.7e$+$0 & 1.3e$+$0 & 3.3e$-$2 & 1.5e$+$0 & 1.9e$+$1 &  \textbf{0.0}  & 3.3e$+$1 &  \textbf{0.0}  \\
\midrule
Avg. & 5.6e$+$0 & 1.2e$+$0 & 4.9e$+$0 & 1.3e$+$0 & 5.0e$+$0 &  \textbf{2.4e$-$1}  & 7.9e$+$0 & 6.5e$-$1 \\


==> tables/min-discm_floating.tex <==
D1 & 19.0 &  \textbf{0.0}  & 19.0 & 0.0064 & 5.7 & 0.096 & 12.0 &  \textbf{0.0}  \\
D2 & 11.0 &  \textbf{0.0}  & 11.0 & 0.38 & 6.0 & 0.0063 & 4.3 &  \textbf{0.0}  \\
D3 & 6.2 &  \textbf{0.0}  & 3.8 & 0.014 & 0.083 &  \textbf{0.0}  & 8.1 &  \textbf{0.0}  \\
D4 & 0.0015 &  \textbf{0.0}  & 0.02 &  \textbf{0.0}  & 3.5 & 0.037 & 2.3 &  \textbf{0.0}  \\
D5 & 0.013 &  \textbf{0.0}  & 0.0046 & 0.11 & 0.87 &  \textbf{0.0}  & 0.34 &  \textbf{0.0}  \\
D6 & 0.045 &  \textbf{0.0}  & 0.0046 & 0.02 & 0.16 & 0.00098 & 0.01 &  \textbf{0.0}  \\
D7 & 1.2 &  \textbf{0.0}  & 0.04 & 0.65 & 1.3 &  \textbf{0.0}  & 0.046 &  \textbf{0.0}  \\
D8 & 0.019 &  \textbf{0.0}  &  \textbf{0.0}  & 0.019 & 19.0 &  \textbf{0.0}  & 33.0 &  \textbf{0.0}  \\
\midrule
Avg. & 4.7 &  \textbf{0.0}  & 4.2 & 0.15 & 4.6 & 0.018 & 7.5 &  \textbf{0.0}  \\


==> tables/min-discm_scientific.tex <==
D1 & 1.9e$+$1 &  \textbf{0.0}  & 1.9e$+$1 & 6.4e$-$3 & 5.7e$+$0 & 9.6e$-$2 & 1.2e$+$1 &  \textbf{0.0}  \\
D2 & 1.1e$+$1 &  \textbf{0.0}  & 1.1e$+$1 & 3.8e$-$1 & 6.0e$+$0 & 6.3e$-$3 & 4.3e$+$0 &  \textbf{0.0}  \\
D3 & 6.2e$+$0 &  \textbf{0.0}  & 3.8e$+$0 & 1.4e$-$2 & 8.3e$-$2 &  \textbf{0.0}  & 8.1e$+$0 &  \textbf{0.0}  \\
D4 & 1.5e$-$3 &  \textbf{0.0}  & 2.0e$-$2 &  \textbf{0.0}  & 3.5e$+$0 & 3.7e$-$2 & 2.3e$+$0 &  \textbf{0.0}  \\
D5 & 1.3e$-$2 &  \textbf{0.0}  & 4.6e$-$3 & 1.1e$-$1 & 8.7e$-$1 &  \textbf{0.0}  & 3.4e$-$1 &  \textbf{0.0}  \\
D6 & 4.5e$-$2 &  \textbf{0.0}  & 4.6e$-$3 & 2.0e$-$2 & 1.6e$-$1 & 9.8e$-$4 & 1.0e$-$2 &  \textbf{0.0}  \\
D7 & 1.2e$+$0 &  \textbf{0.0}  & 4.0e$-$2 & 6.5e$-$1 & 1.3e$+$0 &  \textbf{0.0}  & 4.6e$-$2 &  \textbf{0.0}  \\
D8 & 1.9e$-$2 &  \textbf{0.0}  &  \textbf{0.0}  & 1.9e$-$2 & 1.9e$+$1 &  \textbf{0.0}  & 3.3e$+$1 &  \textbf{0.0}  \\
\midrule
Avg. & 4.7e$+$0 &  \textbf{0.0}  & 4.2e$+$0 & 1.5e$-$1 & 4.6e$+$0 & 1.8e$-$2 & 7.5e$+$0 &  \textbf{0.0}  \\


==> tables/min-parity-diff_debiasedtest.tex <==
D1 & 21.0 & 9.0 & 20.0 & 5.5 & 0.00024 & 0.0095 & 3.1 & 14.0  \\  
D2 & 14.0 & 6.7 & 13.0 & 4.7 & 0.14 & 0.0035 & 0.099 & 7.4  \\  
D3 & 1.5 & 0.6 & 0.62 & 0.079 & 0.25 & 0.14 & 0.19 & 0.016  \\  
D4 & 1.5 & 0.39 & 0.36 & 0.39 & 0.34 & 1.4 & 0.66 & 0.39  \\  
D5 & 0.011 & 0.28 & 0.86 & 0.083 & 12.0 & 0.0 & 1.4 & 0.32  \\  
D6 & 0.2 & 12.0 & 42.0 & 16.0 & 30.0 & 0.0 & 0.51 & 13.0  \\  
D7 & 6.7 & 0.33 & 6.3 & 0.17 & 2.6 & 0.0 & 2.3 & 0.033  \\  
D8 & 5.0 & 5.0 & 5.0 & 5.0 & 5.0 & 0.0 & 0.0 & 5.0  \\  \midrule


==> tables/min-parity-diff_fulltest.tex <==
D1 & 28 & 12 & 27 & 8.7 &  \textbf{0.013}  &  \textbf{0.013}  & 0.18 & 7.1 \\
D2 & 18 & 7.9 & 18 & 5 & 0.28 &  \textbf{0.0024}  & 0.37 & 7.6 \\
D3 & 0.32 & 0.22 & 0.026 & 0.25 &  \textbf{0.0}  &  \textbf{0.0}  & 0.19 & 0.016 \\
D4 & 0.27 &  \textbf{0.075}  & 0.39 &  \textbf{0.075}  & 0.077 & 0.15 & 1.1 &  \textbf{0.075}  \\
D5 & 20 & 17 & 26 & 0.019 & 0.011 &  \textbf{0.0}  & 0.96 & 12 \\
D6 & 33 & 19 & 42 & 9.6 &  \textbf{0.0013}  & 18 & 5.5 & 16 \\
D7 & 8.9 & 3 & 8.3 & 0.022 & 0.14 &  \textbf{0.0}  & 0.62 & 0.12 \\
D8 &  \textbf{0.0}  &  \textbf{0.0}  &  \textbf{0.0}  &  \textbf{0.0}  &  \textbf{0.0}  &  \textbf{0.0}  &  \textbf{0.0}  &  \textbf{0.0}  \\
\midrule
Avg. & 14 & 7.4 & 15 & 3 &  \textbf{0.065}  & 2.3 & 1.1 & 5.4 \\


==> tables/min-parity-diff_fulltest_dist10.tex <==
D1 & 28 & 12 & 27 & 8.7 &  \textbf{0.013}  &  \textbf{0.013}  & 0.18 & 8.8 \\
D2 & 18 & 7.9 & 18 & 5 & 0.28 &  \textbf{0.0024}  & 0.37 & 9 \\
D3 & 0.32 & 0.22 & 0.026 & 0.25 &  \textbf{0.0}  &  \textbf{0.0}  & 0.19 & 0.095 \\
D4 & 0.27 &  \textbf{0.075}  & 0.39 &  \textbf{0.075}  & 0.077 & 0.15 & 1.1 &  \textbf{0.075}  \\
D5 & 20 & 17 & 26 & 0.019 & 0.011 &  \textbf{0.0}  & 0.96 & 0.044 \\
D6 & 33 & 19 & 42 & 9.6 &  \textbf{0.0013}  & 18 & 5.5 & 17 \\
D7 & 8.9 & 3 & 8.3 & 0.022 & 0.14 &  \textbf{0.0}  & 0.62 & 6.5 \\
D8 &  \textbf{0.0}  &  \textbf{0.0}  &  \textbf{0.0}  &  \textbf{0.0}  &  \textbf{0.0}  &  \textbf{0.0}  &  \textbf{0.0}  &  \textbf{0.0}  \\
\midrule
Avg. & 14 & 7.4 & 15 & 3 &  \textbf{0.065}  & 2.3 & 1.1 & 5.2 \\


==> tables/min-parity-model_dist10_scientific.tex <==
D1 & 2.0e$+$1 & 1.1e$-$1 & 2.0e$+$1 &  \textbf{1.0e$-$1}  & 6.7e$+$0 & 5.2e$+$0 & 1.7e$+$1 & 7.5e$-$1 
& 81 & 84 & 82 &  \textbf{85}  & 81 & 82 &  \textbf{85}  &  \textbf{85}  
& 28 & 12 & 27 & 8.7 &  \textbf{0.013}  &  \textbf{0.013}  & 0.18 & 8.8 \\
D2 & 1.3e$+$1 &  \textbf{2.2e$-$1}  & 1.3e$+$1 & 1.8e$+$0 & 7.5e$+$0 & 1.1e$+$0 & 5.3e$+$0 & 1.2e$+$0 
& 79 & 79 & 80 & 80 & 79 & 79 &  \textbf{87}  & 81 
& 18 & 7.9 & 18 & 5 & 0.28 &  \textbf{0.0024}  & 0.37 & 9 \\
D3 & 7.8e$+$0 & 2.6e$+$0 & 9.1e$+$0 & 3.0e$+$0 & 3.3e$+$0 &  \textbf{1.5e$+$0}  & 9.5e$+$0 & 2.8e$+$0 
& 79 &  \textbf{82}  & 75 & 77 & 71 & 73 & 80 & 78 
& 0.32 & 0.22 & 0.026 & 0.25 &  \textbf{0.0}  &  \textbf{0.0}  & 0.19 & 0.095 \\
D4 & 6.0e$+$0 & 5.3e$+$0 & 5.9e$+$0 & 5.4e$+$0 & 7.2e$+$0 & 5.9e$+$0 & 6.2e$+$0 &  \textbf{4.2e$+$0}  
&  \textbf{99}  &  \textbf{99}  &  \textbf{99}  &  \textbf{99}  & 97 & 79 & 98 &  \textbf{99}  
& 0.27 &  \textbf{0.075}  & 0.39 &  \textbf{0.075}  & 0.077 & 0.15 & 1.1 &  \textbf{0.075}  \\
D5 & 3.2e$-$1 & 4.1e$-$1 & 2.1e$-$2 & 2.8e$-$1 & 1.7e$+$0 &  \textbf{0.0}  & 3.8e$-$1 & 9.8e$-$5 
& 63 & 64 & 62 & 44 & 72 & 70 & 65 &  \textbf{100}  
& 20 & 17 & 26 & 0.019 & 0.011 &  \textbf{0.0}  & 0.96 & 0.044 \\
D6 & 5.2e$-$2 & 6.1e$-$2 & 8.8e$-$3 & 5.8e$-$2 & 3.1e$-$1 & 4.6e$-$1 & 1.4e$-$2 &  \textbf{2.3e$-$4}  
& 66 & 70 & 48 & 64 & 78 & 70 & 74 &  \textbf{99}  
& 33 & 19 & 42 & 9.6 &  \textbf{0.0013}  & 18 & 5.5 & 17 \\
D7 & 2.1e$+$0 & 1.9e$+$0 & 4.6e$-$1 & 1.9e$+$0 & 2.2e$+$0 &  \textbf{0.0}  & 6.5e$-$1 &  \textbf{0.0}  
& 76 & 75 & 73 & 78 & 78 &  \textbf{86}  & 84 & 81 
& 8.9 & 3 & 8.3 & 0.022 & 0.14 &  \textbf{0.0}  & 0.62 & 6.5 \\
D8 & 1.7e$+$0 & 1.3e$+$0 & 2.2e$+$0 & 1.5e$+$0 & 2.5e$+$1 &  \textbf{0.0}  & 3.3e$+$1 & 8.6e$-$1 
&  \textbf{100}  &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  & 75 &  \textbf{100}  
&  \textbf{0.0}  &  \textbf{0.0}  &  \textbf{0.0}  &  \textbf{0.0}  &  \textbf{0.0}  &  \textbf{0.0}  &  \textbf{0.0}  &  \textbf{0.0}  \\
\midrule
Avg. & 6.4e$+$0 & 1.5e$+$0 & 6.3e$+$0 & 1.8e$+$0 & 6.7e$+$0 & 1.8e$+$0 & 9.0e$+$0 &  \textbf{1.2e$+$0}  
& 80 & 81 & 77 & 78 & 82 & 79 & 81 &  \textbf{90}  
& 14 & 7.4 & 15 & 3 &  \textbf{0.065}  & 2.3 & 1.1 & 5.2 \\


==> tables/min-parity-model_scientific.tex <==
D1 & 2.0e$+$1 &  \textbf{0.0}  & 2.0e$+$1 & 1.0e$-$1 & 6.7e$+$0 & 5.2e$+$0 & 1.7e$+$1 & 2.2e$-$05 
& 81 & 81 & 81 & 81 & 80 & 82 & 85 &  \textbf{92}  
& 28 & 12 & 27 & 8.7 &  \textbf{0.013}  &  \textbf{0.013}  & 0.18 & 7.1 \\
D2 & 1.3e$+$1 &  \textbf{0.0}  & 1.3e$+$1 & 1.8e$+$0 & 7.5e$+$0 & 2.5e$-$2 & 5.3e$+$0 & 4.2e$-$4 
& 84 & 84 & 85 & 85 & 84 & 84 & 88 &  \textbf{91}  
& 18 & 7.9 & 18 & 5 & 0.28 &  \textbf{0.0024}  & 0.37 & 7.6 \\
D3 & 7.6e$+$0 &  \textbf{0.0}  & 9.1e$+$0 & 2.0e$+$0 & 1.2e$+$0 & 3.9e$-$1 & 9.1e$+$0 & 2.4e$-$1 
& 78 &  \textbf{82}  & 76 & 76 & 71 & 72 & 80 & 74 
& 0.32 & 0.22 & 0.026 & 0.25 &  \textbf{0.0}  &  \textbf{0.0}  & 0.19 & 0.016 \\
D4 & 3.9e$+$0 &  \textbf{0.0}  & 3.6e$+$0 & 1.2e$+$0 & 7.1e$+$0 & 5.5e$+$0 & 4.6e$+$0 & 4.6e$-$3 
& 93 &  \textbf{96}  & 92 & 93 & 90 & 77 & 89 & 94 
& 0.27 &  \textbf{0.075}  & 0.39 &  \textbf{0.075}  & 0.077 & 0.15 & 1.1 &  \textbf{0.075}  \\
D5 & 8.5e$-$2 &  \textbf{0.0}  & 1.4e$-$2 & 2.4e$-$1 & 1.5e$+$0 &  \textbf{0.0}  & 3.4e$-$1 & 5.9e$-$3 
& 67 & 75 & 64 & 44 & 81 & 73 & 76 &  \textbf{100}  
& 20 & 17 & 26 & 0.019 & 0.011 &  \textbf{0.0}  & 0.96 & 12 \\
D6 & 4.9e$-$2 &  \textbf{0.0}  & 8.3e$-$3 & 3.2e$-$2 & 2.5e$-$1 & 4.1e$-$2 & 1.3e$-$2 & 2.1e$-$3 
& 72 & 78 & 48 & 68 & 82 & 71 & 77 &  \textbf{100}  
& 33 & 19 & 42 & 9.6 &  \textbf{0.0013}  & 18 & 5.5 & 16 \\
D7 & 1.2e$+$0 &  \textbf{0.0}  & 7.1e$-$2 & 9.8e$-$1 & 1.4e$+$0 &  \textbf{0.0}  & 4.9e$-$1 &  \textbf{0.0}  
& 76 & 77 & 73 & 77 & 78 & 83 &  \textbf{84}  & 77 
& 8.9 & 3 & 8.3 & 0.022 & 0.14 &  \textbf{0.0}  & 0.62 & 0.12 \\
D8 & 1.0e$+$0 &  \textbf{0.0}  & 2.2e$+$0 & 3.8e$-$2 & 2.5e$+$1 &  \textbf{0.0}  & 3.3e$+$1 &  \textbf{0.0}  
&  \textbf{100}  &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  & 71 &  \textbf{100}  
&  \textbf{0.0}  &  \textbf{0.0}  &  \textbf{0.0}  &  \textbf{0.0}  &  \textbf{0.0}  &  \textbf{0.0}  &  \textbf{0.0}  &  \textbf{0.0}  \\
\midrule
Avg. & 5.9e$+$0 &  \textbf{0.0}  & 6.0e$+$0 & 8.0e$-$1 & 6.3e$+$0 & 1.4e$+$0 & 8.7e$+$0 & 3.2e$-$2 
& 81 & 84 & 77 & 78 & 83 & 80 & 81 &  \textbf{91}  
& 14 & 7.4 & 15 & 3 &  \textbf{0.065}  & 2.3 & 1.1 & 5.4 \\


==> tables/parity-diff-max-accuracy_debiasedtest.tex <==
D1 & 22.0 & 10.0 & 22.0 & 7.9 & 1.0 & 0.2 & 3.1 & 15.0  \\  
D2 & 16.0 & 6.8 & 15.0 & 8.3 & 4.7 & 0.36 & 4.2 & 13.0  \\  
D3 & 15.0 & 6.5 & 15.0 & 6.1 & 4.7 & 1.0 & 3.7 & 7.9  \\  
D4 & 17.0 & 7.0 & 9.2 & 5.7 & 12.0 & 16.0 & 14.0 & 17.0  \\  
D5 & 7.6 & 6.7 & 16.0 & 3.8 & 21.0 & 17.0 & 21.0 & 32.0  \\  
D6 & 3.7 & 26.0 & 48.0 & 29.0 & 40.0 & 1.8 & 2.3 & 34.0  \\  
D7 & 11.0 & 3.3 & 7.4 & 0.35 & 4.1 & 0.86 & 2.7 & 4.5  \\  
D8 & 10.0 & 10.0 & 10.0 & 10.0 & 10.0 & 33.0 & 0.0 & 10.0  \\  \midrule


==> tables/parity-diff-max-accuracy_fulltest.tex <==
D1 & 29 & 13 & 29 & 11 & 1.5 & 3.3 &  \textbf{0.18}  & 9.9 \\
D2 & 22 & 13 & 21 & 11 & 5.4 &  \textbf{0.18}  & 0.37 & 13 \\
D3 & 11 & 3.1 & 6.1 & 3.2 &  \textbf{1.2}  & 2.6 & 5 & 7.9 \\
D4 & 18 & 5.7 & 20 &  \textbf{2.4}  & 8 & 16 & 12 & 17 \\
D5 & 32 & 26 & 38 & 3.9 &  \textbf{1.6}  & 21 & 22 & 26 \\
D6 & 38 & 25 & 48 & 15 &  \textbf{0.078}  & 22 & 26 & 26 \\
D7 & 13 & 6.1 & 9 & 2.1 &  \textbf{1.2}  & 2 & 2.3 & 3.4 \\
D8 & 11 & 11 & 10 & 10 &  \textbf{0.0}  & 12 &  \textbf{0.0}  & 10 \\
\midrule
Avg. & 22 & 13 & 23 & 7.3 &  \textbf{2.4}  & 9.9 & 8.5 & 14 \\


==> tables/parity-diff-max-accuracy_fulltest_dist10.tex <==
D1 & 29 & 13 & 29 & 11 & 1.5 & 3.3 &  \textbf{0.18}  & 12 \\
D2 & 22 & 13 & 21 & 11 & 5.4 &  \textbf{0.18}  & 0.37 & 14 \\
D3 & 11 & 3.1 & 6.1 & 3.2 &  \textbf{1.2}  & 2.6 & 5 & 5.8 \\
D4 & 18 & 5.7 & 20 &  \textbf{2.4}  & 8 & 16 & 12 & 16 \\
D5 & 32 & 26 & 38 & 3.9 &  \textbf{1.6}  & 21 & 22 & 28 \\
D6 & 38 & 25 & 48 & 15 &  \textbf{0.078}  & 22 & 26 & 19 \\
D7 & 13 & 6.1 & 9 & 2.1 &  \textbf{1.2}  & 2 & 2.3 & 12 \\
D8 & 11 & 11 & 10 & 10 &  \textbf{0.0}  & 12 &  \textbf{0.0}  & 10 \\
\midrule
Avg. & 22 & 13 & 23 & 7.3 &  \textbf{2.4}  & 9.9 & 8.5 & 15 \\


==> tables/parity-diff-min-discm_debiasedtest.tex <==
D1 & 22.0 & 10.0 & 21.0 & 6.1 & 2.2 & 0.36 & 4.4 & 15.0  \\  
D2 & 15.0 & 6.8 & 15.0 & 9.0 & 7.1 & 0.0035 & 4.6 & 11.0  \\  
D3 & 7.1 & 6.5 & 7.2 & 13.0 & 11.0 & 1.1 & 0.32 & 9.8  \\  
D4 & 19.0 & 7.0 & 22.0 & 14.0 & 13.0 & 5.2 & 19.0 & 30.0  \\  
D5 & 1.6 & 6.7 & 13.0 & 1.1 & 15.0 & 0.0 & 20.0 & 2.7  \\  
D6 & 1.8 & 26.0 & 49.0 & 22.0 & 32.0 & 15.0 & 11.0 & 14.0  \\  
D7 & 10.0 & 3.3 & 9.1 & 1.3 & 6.9 & 0.0 & 4.3 & 0.033  \\  
D8 & 55.0 & 10.0 & 33.0 & 50.0 & 57.0 & 0.0 & 0.0 & 47.0  \\  \midrule


==> tables/parity-diff-min-discm_fulltest.tex <==
D1 & 29 & 13 & 28 & 8.7 & 3.3 & 3.6 &  \textbf{2.3}  & 7.8 \\
D2 & 21 & 13 & 20 & 12 & 7 &  \textbf{0.33}  & 7.8 & 10 \\
D3 & 1.6 & 3.1 & 2.1 & 14 & 6.2 &  \textbf{0.085}  & 1.5 & 9.8 \\
D4 & 15 & 5.7 & 20 & 12 & 13 &  \textbf{3.8}  & 11 & 25 \\
D5 & 21 & 26 & 33 & 2.3 & 3.7 &  \textbf{0.0}  & 0.96 & 25 \\
D6 & 39 & 25 & 49 & 14 &  \textbf{1.1}  & 22 & 26 & 23 \\
D7 & 12 & 6.1 & 11 & 1.6 & 4.6 &  \textbf{0.0}  & 3.4 & 0.12 \\
D8 & 33 & 11 & 12 & 22 & 50 &  \textbf{0.0}  &  \textbf{0.0}  &  \textbf{0.0}  \\
\midrule
Avg. & 21 & 13 & 22 & 11 & 11 &  \textbf{3.7}  & 6.6 & 13 \\


==> tables/parity-diff-min-discm_fulltest_dist10.tex <==
D1 & 29 & 15 & 28 & 8.9 & 3.3 & 3.6 &  \textbf{2.3}  & 9.8 \\
D2 & 21 & 8.1 & 20 & 12 & 7 &  \textbf{0.59}  & 7.8 & 12 \\
D3 & 1.6 &  \textbf{1.1}  & 2.1 & 2.1 & 3.3 & 2.7 & 1.5 & 7.6 \\
D4 & 13 & 12 & 6.6 & 13 & 12 & 5.4 & 11 &  \textbf{4.4}  \\
D5 & 26 & 24 & 33 & 2.4 & 3.7 &  \textbf{0.0}  & 8.4 & 0.72 \\
D6 & 38 & 23 & 47 & 14 &  \textbf{1.1}  & 21 & 26 & 26 \\
D7 & 12 & 4.7 & 11 & 1.4 & 4.6 &  \textbf{0.0}  & 3.4 & 6.5 \\
D8 &  \textbf{0.0}  &  \textbf{0.0}  & 30 &  \textbf{0.0}  & 50 &  \textbf{0.0}  &  \textbf{0.0}  & 30 \\
\midrule
Avg. & 18 & 11 & 22 & 6.7 & 11 &  \textbf{4.2}  & 7.5 & 12 \\


==> tables/parity-diff-overall.tex <==
D1 & 28.0 & 12.0 & 27.0 & 8.7 & \textbf{0.013} & \textbf{0.013} & 0.18 & 7.1 & 29.0 & 13.0 & 29.0 & 11.0 & 1.5 & 3.3 & \textbf{0.18} & 9.9  \\  
D2 & 18.0 & 7.9 & 18.0 & 5.0 & 0.28 & \textbf{0.0024} & 0.37 & 7.6 & 22.0 & 13.0 & 21.0 & 11.0 & 5.4 & \textbf{0.18} & 0.37 & 13.0  \\  
D3 & 0.32 & 0.22 & 0.026 & 0.25 & \textbf{0.0} & \textbf{0.0} & 0.19 & 0.016 & 11.0 & 3.1 & 6.1 & 3.2 & \textbf{1.2} & 2.6 & 5.0 & 7.9  \\  
D4 & 0.27 & \textbf{0.075} & 0.39 & \textbf{0.075} & 0.077 & 0.15 & 1.1 & \textbf{0.075} & 18.0 & 5.7 & 20.0 & \textbf{2.4} & 8.0 & 16.0 & 12.0 & 17.0  \\  
D5 & 20.0 & 17.0 & 26.0 & 0.019 & 0.011 & \textbf{0.0} & 0.96 & 12.0 & 32.0 & 26.0 & 38.0 & 3.9 & \textbf{1.6} & 21.0 & 22.0 & 26.0  \\  
D6 & 33.0 & 19.0 & 42.0 & 9.6 & \textbf{0.0013} & 18.0 & 5.5 & 16.0 & 38.0 & 25.0 & 48.0 & 15.0 & \textbf{0.078} & 22.0 & 26.0 & 26.0  \\  
D7 & 8.9 & 3.0 & 8.3 & 0.022 & 0.14 & \textbf{0.0} & 0.62 & 0.12 & 13.0 & 6.1 & 9.0 & 2.1 & \textbf{1.2} & 2.0 & 2.3 & 3.4  \\  
D8 & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & 11.0 & 11.0 & 10.0 & 10.0 & \textbf{0.0} & 12.0 & \textbf{0.0} & 10.0  \\  \midrule
Avg. & 13.6 & 7.40 & 15.2 & 2.96 & \textbf{0.0653} & 2.27 & 1.11 & 5.36 & 21.8 & 12.9 & 22.6 & 7.33 & \textbf{2.37} & 9.88 & 8.48 & 14.20 \\

==> tables/test_accuracy_for_min_discm.tex <==
D1 & 80 & 82 & 80 & 81 & 80 & 81 & 85 &  \textbf{92}  \\
D2 & 83 & 85 & 84 & 84 & 83 & 84 & 87 &  \textbf{92}  \\
D3 & 75 &  \textbf{82}  & 74 & 73 & 75 & 62 & 76 & 81 \\
D4 & 96 &  \textbf{98}  & 95 & 92 & 92 & 69 & 92 & 96 \\
D5 & 73 &  \textbf{77}  & 62 & 48 & 76 & 73 & 76 & 74 \\
D6 & 67 & 81 & 49 & 65 & 78 & 78 & 79 &  \textbf{84}  \\
D7 & 76 & 78 & 71 & 77 & 75 & 83 &  \textbf{85}  & 80 \\
D8 &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  & 50 & 75 &  \textbf{100}  \\
\midrule
Avg. & 81 & 85 & 76 & 77 & 82 & 72 & 81 &  \textbf{87}  \\


==> tables/test_accuracy_for_min_discm_dist10.tex <==
D1 & 81 & 83 & 81 & 85 & 81 & 84 & 85 &  \textbf{86}  \\
D2 & 79 & 80 & 80 & 80 & 79 & 80 &  \textbf{85}  & 81 \\
D3 & 75 & 81 & 74 & 73 & 76 & 62 & 76 &  \textbf{82}  \\
D4 & 99 & 98 &  \textbf{100}  & 98 & 96 & 90 & 98 & 97 \\
D5 & 63 & 62 & 60 & 44 & 63 & 70 & 64 &  \textbf{100}  \\
D6 & 60 & 67 & 49 & 59 & 72 & 72 & 67 &  \textbf{99}  \\
D7 & 76 & 76 & 71 & 76 & 75 &  \textbf{86}  & 85 & 83 \\
D8 &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  & 57 & 75 &  \textbf{100}  \\
\midrule
Avg. & 79 & 80 & 76 & 76 & 80 & 75 & 79 &  \textbf{91}  \\


==> tables/test_accuracy_for_min_parity.tex <==
D1 & 81 & 81 & 81 & 81 & 80 & 82 & 85 &  \textbf{92}  \\
D2 & 84 & 84 & 85 & 85 & 84 & 84 & 88 &  \textbf{91}  \\
D3 & 78 &  \textbf{82}  & 76 & 76 & 71 & 72 & 80 & 74 \\
D4 & 93 &  \textbf{96}  & 92 & 93 & 90 & 77 & 89 & 94 \\
D5 & 67 & 75 & 64 & 44 & 81 & 73 & 76 &  \textbf{100}  \\
D6 & 72 & 78 & 48 & 68 & 82 & 71 & 77 &  \textbf{100}  \\
D7 & 76 & 77 & 73 & 77 & 78 & 83 &  \textbf{84}  & 77 \\
D8 &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  & 71 &  \textbf{100}  \\
\midrule
Avg. & 81 & 84 & 77 & 78 & 83 & 80 & 81 &  \textbf{91}  \\


==> tables/test_accuracy_for_min_parity_dist10.tex <==
D1 & 81 & 84 & 82 &  \textbf{85}  & 81 & 82 &  \textbf{85}  &  \textbf{85}  \\
D2 & 79 & 79 & 80 & 80 & 79 & 79 &  \textbf{87}  & 81 \\
D3 & 79 &  \textbf{82}  & 75 & 77 & 71 & 73 & 80 & 78 \\
D4 &  \textbf{99}  &  \textbf{99}  &  \textbf{99}  &  \textbf{99}  & 97 & 79 & 98 &  \textbf{99}  \\
D5 & 63 & 64 & 62 & 44 & 72 & 70 & 65 &  \textbf{100}  \\
D6 & 66 & 70 & 48 & 64 & 78 & 70 & 74 &  \textbf{99}  \\
D7 & 76 & 75 & 73 & 78 & 78 &  \textbf{86}  & 84 & 81 \\
D8 &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  &  \textbf{100}  & 75 &  \textbf{100}  \\
\midrule
Avg. & 80 & 81 & 77 & 78 & 82 & 79 & 81 &  \textbf{90}  \\

